ResoFilter: Fine-grained Synthetic Data Filtering for Large Language Models through Data-Parameter Resonance Analysis

Large language models (LLMs) have shown remarkable effectiveness across various domains, with data augmentation methods utilizing GPT for synthetic data generation becoming prevalent. However, the quality and utility of augmented data remain questionable, and current methods lack clear metrics for evaluating data characteristics. To address these challenges, we propose ResoFilter, a novel method that integrates models, data, and tasks to refine datasets. ResoFilter leverages the fine-tuning process to obtain Data-Parameter features for data selection, offering improved interpretability by representing data characteristics through model weights. Our experiments demonstrate that ResoFilter achieves comparable results to full-scale fine-tuning using only half the data in mathematical tasks and exhibits strong generalization across different models and domains. This method provides valuable insights for constructing synthetic datasets and evaluating high-quality data, offering a promising solution for enhancing data augmentation techniques and improving training dataset quality for LLMs. For reproducibility, we will release our code and data upon acceptance.

==> latex/mxd/task_wise.tex <==
\begin{figure}[!t]
  \centering
  \resizebox{0.45\textwidth}{!}{
    % \includegraphics{img/pipeline_1.png}
    \includegraphics{img/distri_multi.pdf}
  }
  \vspace{-5pt}
  \caption{Under the analysis of our method, the distribution of tasks in the dataset can be clearly observed.}
  \label{dis}
  \vspace{1pt}
\end{figure}


==> latex/tza/table/res_benchmark.tex <==
\begin{table}[t!]
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|l|ccc|c}
    \toprule
    \textbf{Fields} & \textbf{Method} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} & \textbf{Full SFT} \\
    \midrule
    \multirow{3}{*}{CodeX} 
    & Random & 0.2979 & 0.3549 & \textbf{0.404} & \multirow{3}{*}{0.4098}\\
    & Loss & 0.3146 & 0.3442 & 0.3872 & \\
    & Our method & \textbf{0.3579} & \textbf{0.425} & 0.3966 & \\
    \midrule
    \multirow{3}{*}{MMLU} 
    & Random & 0.5105 & \textbf{0.5152} & 0.4858 & \multirow{3}{*}{0.4658}\\
    & Loss & 0.507 & 0.501 & \textbf{0.4961} & \\
    & Our method & \textbf{0.5129} & 0.4893 & 0.4952 & \\
    \midrule
    \multirow{3}{*}{BBH} 
    & Random & 0.3796 & \textbf{0.3759} & \textbf{0.3824} & \multirow{3}{*}{0.3704}\\
    & Loss & 0.3796 & 0.3667 & 0.3685 & \\
    & Our method & \textbf{0.3861} & 0.362 & 0.3778 & \\
    \bottomrule
    \end{tabular}}
    \caption{Cross-domain evaluation results comparing our proposed method with random sampling. There has been significant improvement in code generation while in general domain it is not obvious. We have more detail experiments and explanations in Appendix~\ref{mmlu_analysis}}
    \label{res_bench}
\end{table}



==> latex/tza/table/res_model.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{l|l|cccc|c}
    \toprule
    \textbf{Model} & \textbf{Method} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} & \textbf{Full SFT} & \textbf{Time Cost(Hour)} \\
    \midrule
    \multirow{6}{*}{Gemma2-2B} 
    & Random & 0.6042 & 0.6254 & 0.6474 & \multirow{6}{*}{0.649} & - \\
    & Loss & 0.6034 & 0.6436 & 0.6436 & & 0.8 \\
    & PPL & 0.6035 & 0.6467 & 0.655 & & 0.8 \\
    & Superfiltering & 0.5079 & 0.6262 & 0.6482 & & 0.8 \\
    & Nuggest & 0.5565 & 0.6164 & 0.6543 & & \textbf{98} \\
    & Our method & \textbf{0.6042} & \textbf{0.6497} & \textbf{0.6603} & & 1.5 \\
    \midrule
    \multirow{5}{*}{Llama2-7B} 
    & Random & 0.5525 & 0.5921 & 0.5981 & \multirow{5}{*}{0.5731} & - \\
    & Loss & 0.5034 & 0.5413 & 0.5459 & & 1.7 \\
    & PPL & 0.511 & 0.5353 & 0.5451 & & 1.7 \\
    & Superfiltering & 0.3972 & 0.6073 & \textbf{0.6531} & & 2 \\
    & Our method & \textbf{0.5549} & \textbf{0.6196} & 0.6444 & & 4.5 \\
    \midrule
    \multirow{5}{*}{Llama2-13B} 
    & Random & 0.6276 & 0.6747 & 0.6686 & \multirow{5}{*}{0.6935} & - \\
    & Loss & 0.6096 & 0.6209 & 0.6641 & & 4.9 \\
    & PPL & 0.6141 & 0.6338 & 0.6611 & & 4.9 \\
    & Superfiltering & 0.5496 & 0.677 & 0.6831 & & 5.5 \\
    & Our method & \textbf{0.6322} & \textbf{0.6853} & \textbf{0.6855} & & 9 \\
    \bottomrule
    \end{tabular}}
    \caption{Figure~\ref{res_model} presents a comprehensive comparison of our proposed method against several baseline approaches across three different model architectures: Gemma2-2B, Llama2-7B, and Llama2-13B.  In addition to the three most commonly used types of methods, we also cited two methods for data selection~\cite{li-etal-2024-one}~\cite{li2024superfiltering}. As can be seen, our performance has achieved the best among these methods with only a small increase in time cost compared to other techniques.}
    \label{res_model}
\end{table*}
